Efficient Learning of Locomotion Skills through the Discovery of Diverse Environmental Trajectory Generator Priors

Data-driven learning based methods have recently been particularly successful at learning robust locomotion controllers for a variety of unstructured terrains. Prior work has shown that incorporating good locomotion priors in the form of trajectory generators (TGs) is effective at efficiently learning complex locomotion skills. However, defining a good, single TG as tasks/environments become increasingly more complex remains a challenging problem as it requires extensive tuning and risks reducing the effectiveness of the prior. In this paper, we present Evolved Environmental Trajectory Generators (EETG), a method that learns a diverse set of specialised locomotion priors using Quality-Diversity algorithms while maintaining a single policy within the Policies Modulating TG (PMTG) architecture. The results demonstrate that EETG enables a quadruped robot to successfully traverse a wide range of environments, such as slopes, stairs, rough terrain, and balance beams. Our experiments show that learning a diverse set of specialized TG priors is significantly (5 times) more efficient than using a single, fixed prior when dealing with a wide range of environments.

==> pseudocode.tex <==
% \begin{algorithm} \label{algo:mb-qd}
% \caption{MAP-Elites}
% \begin{algorithmic}[1]
% \State{Initialize repertoire}
%  \\
%  \While{maximum number of evaluations not reached}
%  \\
%   \If{first iteration} \Comment{\textit{Generate random policies at first iteration.}}
%       \State{$\leftarrow$ random\_parameters()}

%   \Else
       
%     \EndIf
%     \\

% \EndWhile
% \end{algorithmic}
% \end{algorithm}


% \begin{algorithm}\label{algo:eetg}
% \caption{MAP-Elites + PMTG Algorithm}\label{alg}
%     \begin{algorithmic}
%         \Require
%         \State $N \gets \text{number of iterations}$
%         \State $M \gets \text{number of iterations of the MAP-Elites (ME)}$
%         \State $P \gets \text{number of iterations for the PMTG Loop}$
%         \State $B \gets \text{batch size at each ME generation}$
%         \State $E \gets \text{maximum length of an episode}$
%         \newline
%         \State $grid \gets \text{MAP-Elites grid that stores all the environments and solutions}$
%         \State $\pi \gets \text{initialise policy weights and biases with 0s}$
%         \State $\alpha \gets \text{learning rate for updating the policy}$
%         \State $\sigma \gets \text{standard deviation of the exploration noise}$
%         \State $n \gets \text{number of directions sampled per iteration}$
%         \State $b \gets \text{number of top-performing directions to use}$
%         \newline
        
%         \Ensure $b < n$
%         \newline
        
%         \State $grid.init()$
%         \newline
        
%         \For{$iter = 1, ..., N$} 
%             \For{$gen = 1, ..., M$}    \Comment{MAP-Elites Loop}
%                 \State $sol, env \gets grid.select()$
%                 \State $sol \gets sol.mutate()$
%                 \State $fitness \gets evaluate(sol, env)$
%                 \State $sol.update(fitness)$
%                 \State $grid.insert(sol, env)$
%             \EndFor
%             \newline
            
%             \For{$ep = 1, ..., P$}  \Comment{PMTG Loop}
%                 \State $sol, env \gets grid.get\_random\_cell()$
%                 \State $\delta \gets policy.sample\_deltas()$
%                 \State $rewards_+ \gets run\_episodes(sol, env, deltas, ``positive")$
%                 \State $rewards_- \gets run\_episodes(sol, env, deltas, ``negative")$
%                 \State $rewards_\sigma = (reward_+ + rewards_-).std()$
%                 \State $rollouts \gets best\_directions(rewards_+, rewards_-, \delta)$
%                 \State $policy.update(rollouts, rewards_\sigma)$
%             \EndFor
%             \newline
            
%             \State $grid.update\_fitness()$
%             \newline
        
%         \EndFor
            
%     \end{algorithmic}
% \end{algorithm}







==> pseudocode_2.tex <==
\begin{algorithm} 
\caption{PMTG Algorithm} \label{algo:pmtg}
    \begin{algorithmic}
        \Require
        \State $P \gets \text{number of iterations for PMTG}$
        \State $G \gets \text{ME grid containing environments and solutions}$
        \State $\pi_\theta \gets \text{initialise policy weights and biases with 0s}$
        \State $n \gets \text{number of directions sampled per iteration}$
        \State $b \gets \text{number of top-performing directions to use}$
        \newline
        
        \Ensure $b < n$
        \newline

            
        \For{$ep = 1, ..., P$} 
            \State $sol, env \gets G.get\_random\_cell()$
            \State $\delta \gets \pi_\theta.sample\_deltas()$
            \State $rewards_+ \gets run\_episodes(sol, env, \delta, ``positive")$
            \State $rewards_- \gets run\_episodes(sol, env, \delta, ``negative")$
            \State $rewards_\sigma = (reward_+ + rewards_-).std()$
            \State $rollouts \gets best\_directions(rewards_+, rewards_-, \delta)$
            \State $\pi_\theta \gets \pi_\theta.update(rollouts, rewards_\sigma)$
        \EndFor
            
    \end{algorithmic}
\end{algorithm}
